ECM modeling and performance tuning of SpMV and Lattice QCD on A64FX

The A64FX CPU is arguably the most powerful Arm-based processor design to date. Although it is a traditional cache-based multicore processor, its peak performance and memory bandwidth rival accelerator devices. A good understanding of its performance features is of paramount importance for developers who wish to leverage its full potential. We present an architectural analysis of the A64FX used in the Fujitsu FX1000 supercomputer at a level of detail that allows for the construction of Execution-Cache-Memory (ECM) performance models for steady-state loops. In the process we identify architectural peculiarities that point to viable generic optimization strategies. After validating the model using simple streaming loops we apply the insight gained to sparse matrix-vector multiplication (SpMV) and the domain wall (DW) kernel from quantum chromodynamics (QCD). For SpMV we show why the CRS matrix storage format is not a good practical choice on this architecture and how the SELL-C-sigma format can achieve bandwidth saturation. For the DW kernel we provide a cache-reuse analysis and show how an appropriate choice of data layout for complex arrays can realize memory-bandwidth saturation in this case as well. A comparison with state-of-the-art high-end Intel Cascade Lake AP and Nvidia V100 systems puts the capabilities of the A64FX into perspective. We also explore the potential for power optimizations using the tuning knobs provided by the Fugaku system, achieving energy savings of about 31% for SpMV and 18% for DW.

==> plots/tikz/qcd/base_version/1_thread.tex <==
\pgfplotstableread[col sep=comma, header=true]{plots/data/QCD/base_version/thread_1_riri.txt}{\file}

\edef\RLMvalue{25}
%\edef\RLMvalueFCC{724}

%\pgfplotstabletypeset[skip rows between index={0}{0}]{\rawFile}{\file}
\newcommand{\strequal}[2]{\pdf@strcmp{#1}{#2}==0}
\begin{tikzpicture}
\begin{axis}
[
xbar,
%axis y line*=left,
height=4cm,
width=\linewidth,
xmajorgrids=true,
xminorgrids=true,
ymajorgrids=false,
yminorgrids=false,
%tick align=inside,
bar width=0.5cm,
%ymin=0,
%ymax=360,
% ymax=2.75,
xmin=0,
xmax=800,
xlabel={Performance [\GFS]},
%minor y tick num=1,
%xtick={2},
%xticklabels={r=1},
%symbolic y coords = {0,1},
symbolic y coords={gcc,fcc},
ytick={gcc,fcc},
yticklabels={GCC, FCC},
%xmax={yask_new_v},
%xtick={base, if, yask_new_v},  % Use this to decide which tickmarks to print
%xticklabels={base, no jumps, integer move},
%xticklabel style={rotate=22},
%enlarge x limits={abs=0.4cm},
%ylabel near ticks,
enlarge y limits  = 0.6,
%enlarge x limits  = 0.02,
%nodes near coords
]
\addplot table[x expr={\thisrow{GF/s}}, y=compiler] {\file};
%coordinates {(\ririGCC,1) (\ririFCC,2)};
%\addplot[blue] coordinates {(\ririFCC,2)};
\end{axis}
\begin{axis}
[
height=4cm,
width=\linewidth,
xmajorgrids=false,
xminorgrids=false,
ymajorgrids=false,
yminorgrids=false,
%%tick align=inside,
xmin=0,
xmax=800,
%%ymax=360,
%%ylabel={MLUP/s},
xtick=\empty,
%%minor y tick num=1,
xticklabels={},
ytick=\empty,
yticklabels={},
%%ylabel near ticks,
]
\addplot[color=red, very thick, mark=none] coordinates{
	(\RLMvalue,0)
	(\RLMvalue,1)
};
\node[red, rotate=270] at (\RLMvalue-20,0.5) {RLM};
%
%% \addplot[color=darkgreen, very thick, mark=none] coordinates{
%%    (0,\phenoECMvalue)
%%   (1,\phenoECMvalue)
%%   };
\end{axis}

\end{tikzpicture}


%\vspace{-1em}

==> plots/tikz/qcd/split_version/48_threads.tex <==
\pgfplotstableread[col sep=comma, header=true]{plots/data/QCD/prefetch_reorder_O1_version/thread_48_riri.txt}{\fileInterleave}

\pgfplotstableread[col sep=comma, header=true]{plots/data/QCD/prefetch_reorder_O1_version/thread_48_rrii.txt}{\fileSplit}
%\pgfplotstabletypeset[skip rows between index={0}{0}]{\rawFile}{\file}
\edef\RLMvalue{741}

\begin{tikzpicture}
\begin{axis}
[
ybar,
%axis y line*=left,
height=6cm,
width=\linewidth,
ymajorgrids=true,
yminorgrids=true,
xmajorgrids=false,
xminorgrids=false,
%tick align=inside,
bar width=0.4cm,
%ymin=0,
%ymax=360,
% ymax=2.75,
ymin=0,
ymax=800,
ylabel={Performance [\GFS]},
%minor y tick num=1,
%xtick={2},
%xticklabels={r=1},
%symbolic y coords = {0,1},
symbolic x coords={gcc,fcc},
xtick={gcc,fcc},
xticklabels={GCC, FCC},
%xmax={yask_new_v},
%xtick={base, if, yask_new_v},  % Use this to decide which tickmarks to print
%xticklabels={base, no jumps, integer move},
%xticklabel style={rotate=22},
%enlarge x limits={abs=0.4cm},
%ylabel near ticks,
enlarge x limits  = 0.6,
legend pos=north west,
legend style={draw=none},
%enlarge x limits  = 0.02,
]
\addplot table[x=compiler, y expr={\thisrow{GF/s}}] {\fileInterleave};
\addplot table[x=compiler, y expr={\thisrow{GF/s}}] {\fileSplit};
%\legend{base, prefetch, prefetch+O1}
%coordinates {(\ririGCC,1) (\ririFCC,2)};
%\addplot[blue] coordinates {(\ririFCC,2)};
\end{axis}
\begin{axis}
[
height=6cm,
width=\linewidth,
xmajorgrids=false,
xminorgrids=false,
ymajorgrids=false,
yminorgrids=false,
%%tick align=inside,
ymin=0,
ymax=800,
%%ymax=360,
%%ylabel={MLUP/s},
xtick=\empty,
%%minor y tick num=1,
xticklabels={},
ytick=\empty,
yticklabels={},
%%ylabel near ticks,
]
\addplot[color=red, very thick, mark=none] coordinates{
	(0,\RLMvalue)
	(1,\RLMvalue)
};
\node[red, rotate=0] at (0.5,700) {RLM};
\end{axis}

\end{tikzpicture}


%\vspace{-1em}

==> plots/tikz/qcd/split_version/48_threads_L2.tex <==
\pgfplotstableread[col sep=comma, header=true]{plots/data/QCD/prefetch_reorder_O1_version/thread_48_riri.txt}{\fileInterleave}

\pgfplotstableread[col sep=comma, header=true]{plots/data/QCD/prefetch_reorder_O1_version/thread_48_rrii.txt}{\fileSplit}


%\pgfplotstableread[col sep=comma, header=true]{plots/data/QCD/prefetch_reorder_version/thread_48_riri.txt}{\fileReorder}

%\pgfplotstabletypeset[skip rows between index={0}{0}]{\rawFile}{\file}
\newcommand{\strequal}[2]{\pdf@strcmp{#1}{#2}==0}
\begin{tikzpicture}
\begin{axis}
[
ybar,
%axis y line*=left,
height=6cm,
width=\linewidth,
ymajorgrids=true,
yminorgrids=true,
xmajorgrids=false,
xminorgrids=false,
%tick align=inside,
bar width=0.4cm,
%ymin=0,
%ymax=360,
% ymax=2.75,
ymin=0,
ylabel={L2 traffic [\BL]},
%minor y tick num=1,
%xtick={2},
%xticklabels={r=1},
%symbolic y coords = {0,1},
symbolic x coords={gcc,fcc},
xtick={gcc,fcc},
xticklabels={GCC, FCC},
y tick label style={/pgf/number format/.cd,
	set thousands separator={},},
%xmax={yask_new_v},
%xtick={base, if, yask_new_v},  % Use this to decide which tickmarks to print
%xticklabels={base, no jumps, integer move},
%xticklabel style={rotate=22},
%enlarge x limits={abs=0.4cm},
%ylabel near ticks,
enlarge x limits  = 0.6,
%enlarge x limits  = 0.02,
]


\addplot table[x=compiler, y expr={(\thisrow{L2_LD}+\thisrow{L2_ST})*1e9/(\thisrow{iter}*\thisrow{grid_volume})}] {\fileInterleave};

\addplot table[x=compiler, y expr={(\thisrow{L2_LD}+\thisrow{L2_ST})*1e9/(\thisrow{iter}*\thisrow{grid_volume})}] {\fileSplit};

%coordinates {(\ririGCC,1) (\ririFCC,2)};
%\addplot[blue] coordinates {(\ririFCC,2)};
\end{axis}
%\begin{axis}
%[
%height=3.8cm,
%width=\linewidth,
%tick align=inside,
%ymin=0,
%ymax=360,
%ylabel={MLUP/s},
%xtick=\empty,
%minor y tick num=1,
%xticklabels={},
%ylabel near ticks,
%]
%\addplot[color=red, very thick, mark=none] coordinates{
%	(0,\ECMvalue)
%	(1,\ECMvalue)
%};

% \addplot[color=darkgreen, very thick, mark=none] coordinates{
%    (0,\phenoECMvalue)
%   (1,\phenoECMvalue)
%   };
%\end{axis}

\end{tikzpicture}


%\vspace{-1em}

==> plots/tikz/qcd/split_version/48_threads_mem.tex <==
\pgfplotstableread[col sep=comma, header=true]{plots/data/QCD/prefetch_reorder_O1_version/thread_48_riri.txt}{\fileInterleave}

\pgfplotstableread[col sep=comma, header=true]{plots/data/QCD/prefetch_reorder_O1_version/thread_48_rrii.txt}{\fileSplit}

%\pgfplotstableread[col sep=comma, header=true]{plots/data/QCD/prefetch_reorder_version/thread_48_riri.txt}{\fileReorder}

%\pgfplotstabletypeset[skip rows between index={0}{0}]{\rawFile}{\file}
\newcommand{\strequal}[2]{\pdf@strcmp{#1}{#2}==0}
\begin{tikzpicture}
\begin{axis}
[
ybar,
%axis y line*=left,
height=6cm,
width=\linewidth,
ymajorgrids=true,
yminorgrids=true,
xmajorgrids=false,
xminorgrids=false,
%tick align=inside,
bar width=0.4cm,
%ymin=0,
%ymax=360,
% ymax=2.75,
ymin=0,
ylabel={Memory traffic [\BL]},
%minor y tick num=1,
%xtick={2},
%xticklabels={r=1},
%symbolic y coords = {0,1},
symbolic x coords={gcc,fcc},
xtick={gcc,fcc},
xticklabels={GCC, FCC},
y tick label style={/pgf/number format/.cd,
	set thousands separator={},},
%xmax={yask_new_v},
%xtick={base, if, yask_new_v},  % Use this to decide which tickmarks to print
%xticklabels={base, no jumps, integer move},
%xticklabel style={rotate=22},
%enlarge x limits={abs=0.4cm},
%ylabel near ticks,
enlarge x limits  = 0.6,
%enlarge x limits  = 0.02,
]

\addplot table[x=compiler, y expr={(\thisrow{Mem_LD}+\thisrow{Mem_ST})*1e9/(\thisrow{iter}*\thisrow{grid_volume})}] {\fileInterleave};

\addplot table[x=compiler, y expr={(\thisrow{Mem_LD}+\thisrow{Mem_ST})*1e9/(\thisrow{iter}*\thisrow{grid_volume})}] {\fileSplit};
%coordinates {(\ririGCC,1) (\ririFCC,2)};
%\addplot[blue] coordinates {(\ririFCC,2)};
\end{axis}
%\begin{axis}
%[
%height=3.8cm,
%width=\linewidth,
%tick align=inside,
%ymin=0,
%ymax=360,
%ylabel={MLUP/s},
%xtick=\empty,
%minor y tick num=1,
%xticklabels={},
%ylabel near ticks,
%]
%\addplot[color=red, very thick, mark=none] coordinates{
%	(0,\ECMvalue)
%	(1,\ECMvalue)
%};

% \addplot[color=darkgreen, very thick, mark=none] coordinates{
%    (0,\phenoECMvalue)
%   (1,\phenoECMvalue)
%   };
%\end{axis}

\end{tikzpicture}


%\vspace{-1em}

==> plots/tikz/qcd/split_version/legend.tex <==
\begin{tikzpicture}
  \centering
  \begin{customlegend}[
      legend columns=2,
      legend style={
      %draw=none,
      %font=\small,
      anchor=north,
      /tikz/every even column/.append style={column sep=0.25cm}},
      legend entries={RIRI (interleave), RRII (split)},% phenomenological ECM},
      ]
    \addlegendimage{draw=blue, area legend, fill=blue!30!white,legend image post style={xscale=0.8,yscale=1.2}}
    \addlegendimage{draw=red, area legend, fill=red!30!white,legend image post style={xscale=0.8,yscale=1.2}}
  \end{customlegend}
\end{tikzpicture}


==> plots/tikz/spmv_microbench/fcc/scaling_csr.tex <==
\begin{tikzpicture}%[y=.2cm, x=.7cm]%,font=\sffamily]
\centering
\begin{axis}[
%%scale only axis,
height=6cm,
width=\linewidth,
grid=both,
tick align=inside,
%%enlarge y limits={value=.1,upper},
%%axis x line*=bottom,
%%axis y line*=left,
%%y axis line style={opacity=0},
%tickwidth=0pt,
%enlarge x limits=true,
xlabel={\# of active cores},
%ylabel={Effective Bandwidth [GB/s]},
ylabel={Performance [\GFS]},
%ylabel={Effective BW [GB/s]},
%%%%%%xlabel style={},
%%%%%%ylabel style={},
%%%%%%x tick label style={},
%%%%%%y tick label style={},
%minor x tick num = 7,
xmin=0,
xmax=48,
ymin=0,
%ymax=295,
%xtick = {0,4,8,12},
%ytick = {0,  10, 20, 30, 40,50},
%ytick = {0,20,40,60,80,100,120,140},
legend pos=north west,
legend style={draw=none},
%label style={font=\small},
%tick label style={font=\small},
]
\addplot[black, mark=*, mark size=1.0pt, %mark options={fill=white},
thick] table[x expr=\thisrowno{0}, y expr=\thisrowno{1}, header=true, col sep=comma] {plots/data/spmv_microbench/fcc/rect_4000_scaling/spmv_C1_u1.dat};
\addlegendentry{TSM-4000}

\addplot[red, mark=none, mark size=1.0pt, %mark options={fill=white},
thick] table[x expr=\thisrowno{0}, y expr=\thisrowno{1}, header=true, col sep=comma] {plots/data/spmv_microbench/fcc/pwtk_scaling/spmv_C1_u1.dat};
\addlegendentry{pwtk}

\end{axis}
%\node[fill=white] at (0.88,2.6) {(a) \textsc{triad}};
\end{tikzpicture}

